A flexible forecasting model for production systems

This paper discusses desirable properties of forecasting models in production systems. It then develops a family of models which are designed to satisfy these properties: highly customizable to capture complex patterns; accommodates a large variety of objectives; has interpretable components; produces robust results; has automatic changepoint detection for trend and seasonality; and runs fast -- making it a good choice for reliable and scalable production systems. The model allows for seasonality at various time scales, events/holidays, and change points in trend and seasonality. The volatility is fitted separately to maintain flexibility and speed and is allowed to be a function of specified features.

==> tables/tables_benchmark_silverkite_config.tex <==
\begin{table}[H]
    \tiny
    \centering
    \begin{tabular}{|c|c|l|}
    \hline
    \multicolumn{1}{|r|}{\multirow{2}{*}{\textbf{Frequency}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Forecast \\ horizon\end{tabular}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Silverkite Template}}}                                                                                                                                                                             \\
    \multicolumn{1}{|r|}{}                                    &                                                                                       & \multicolumn{1}{c|}{}                                                                                                                                                                                                                                                                                                                                                                           \\ \hline
%    \multirow{3}{*}{Hourly}                                   & 1                                                                                     & \begin{tabular}[c]{@{}l@{}}SILVERKITE\_HOURLY\_1 = {[}\\     \# For hourly data, light seasonality up to daily, no trend changepoints,\\     \# together holiday, default feature sets, automatic autoregression and linear fit algorithm.\\     "HOURLY\_SEAS\_LT\_GR\_LINEAR\_CP\_NONE\_HOL\_TG\_FEASET\_ON\_ALGO\_LINEAR\_AR\_AUTO",\\     \# For hourly data, normal seasonality up to daily, light trend changepoints,\\     \# separate holidays +- 4 days, default feature sets, automatic autoregression and linear fit algorithm.\\     "HOURLY\_SEAS\_NM\_GR\_LINEAR\_CP\_LT\_HOL\_SP4\_FEASET\_ON\_ALGO\_LINEAR\_AR\_AUTO",\\     \# For hourly data, light seasonality up to daily, normal trend changepoints,\\     \# separate holidays +- 4 days, no feature sets, automatic autoregression and ridge fit algorithm.\\     "HOURLY\_SEAS\_LT\_GR\_LINEAR\_CP\_NM\_HOL\_SP4\_FEASET\_OFF\_ALGO\_RIDGE\_AR\_AUTO",\\     \# For hourly data, normal seasonality up to daily, normal trend changepoints,\\     \# separate holidays +- 1 day, default feature sets, automatic autoregression and ridge fit algorithm.\\     "HOURLY\_SEAS\_NM\_GR\_LINEAR\_CP\_NM\_HOL\_SP1\_FEASET\_ON\_ALGO\_RIDGE\_AR\_AUTO"\\ {]}\end{tabular}            \\ \cline{2-3}
%                                                              & 24                                                                                    & \begin{tabular}[c]{@{}l@{}}SILVERKITE\_HOURLY\_24 = {[}\\     \# For hourly data, light seasonality up to daily, normal trend changepoints,\\     \# separate holidays +- 4 days, default feature sets, automatic autoregression and ridge fit algorithm.\\     "HOURLY\_SEAS\_LT\_GR\_LINEAR\_CP\_NM\_HOL\_SP4\_FEASET\_ON\_ALGO\_RIDGE\_AR\_AUTO",\\     \# For hourly data, light seasonality up to daily, no trend changepoints,\\     \# separate holidays +- 4 days, default feature sets, automatic autoregression and ridge fit algorithm.\\     "HOURLY\_SEAS\_LT\_GR\_LINEAR\_CP\_NONE\_HOL\_SP4\_FEASET\_ON\_ALGO\_RIDGE\_AR\_AUTO",\\     \# For hourly data, normal seasonality up to daily, light trend changepoints,\\     \# separate holidays +- 1 days, no feature sets, automatic autoregression and linear fit algorithm.\\     "HOURLY\_SEAS\_NM\_GR\_LINEAR\_CP\_LT\_HOL\_SP1\_FEASET\_OFF\_ALGO\_LINEAR\_AR\_AUTO",\\     \# For hourly data, normal seasonality up to daily, normal trend changepoints,\\     \# separate holidays +- 4 day, default feature sets, automatic autoregression and ridge fit algorithm.\\     "HOURLY\_SEAS\_NM\_GR\_LINEAR\_CP\_NM\_HOL\_SP4\_FEASET\_ON\_ALGO\_RIDGE\_AR\_AUTO"\\ {]}\end{tabular} \\ \cline{2-3}
 %                                                             & 24*7                                                                                  &      \\ \hline
    \multirow{3}{*}{Daily}                                    & 1                                                                                     & \begin{tabular}[c]{@{}l@{}}\# For daily data, normal seasonality up to weekly, light trend changepoints,\\ \# separate holidays +- 2 days, default feature sets, and linear fit algorithm.\\ DAILY\_SEAS\_NMQM\_GR\_LINEAR\_CP\_NM\_HOL\_SP2\_FEASET\_AUTO\_ALGO\_RIDGE\_AR\_AUTO\_DSI\_AUTO\_WSI\_AUTO\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                              \\ \cline{2-3}
                                                              & 7                                                                                     & \begin{tabular}[c]{@{}l@{}}\# For daily data, normal seasonality up to weekly, light trend changepoints,\\ \# separate holidays +- 2 days, default feature sets, and linear fit algorithm.\\ DAILY\_SEAS\_NMQM\_GR\_LINEAR\_CP\_NM\_HOL\_SP2\_FEASET\_AUTO\_ALGO\_RIDGE\_AR\_AUTO\_DSI\_AUTO\_WSI\_AUTO\end{tabular}                                                                                                                                                                                                                   \\ \cline{2-3}
%                                                              & 90                                                                                    & \begin{tabular}[c]{@{}l@{}}SILVERKITE\_DAILY\_90 = {[}\\     \# For daily data, light seasonality up to weekly, light trend changepoints,\\     \# separate holidays +- 2 days, default feature sets and linear fit algorithm.\\     "DAILY\_SEAS\_LTQM\_GR\_LINEAR\_CP\_LT\_HOL\_SP2\_FEASET\_AUTO\_ALGO\_LINEAR\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO",\\     \# For daily data, light seasonality up to weekly, no trend changepoints,\\     \# separate holidays +- 2 days, default feature sets and linear fit algorithm.\\     "DAILY\_SEAS\_LTQM\_GR\_LINEAR\_CP\_NONE\_HOL\_SP2\_FEASET\_AUTO\_ALGO\_LINEAR\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO",\\     \# For daily data, light seasonality up to weekly, light trend changepoints,\\     \# separate holidays +- 2 days, default feature sets and ridge fit algorithm.\\     "DAILY\_SEAS\_LTQM\_GR\_LINEAR\_CP\_LT\_HOL\_SP2\_FEASET\_AUTO\_ALGO\_RIDGE\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO",\\     \# For daily data, yearly and weekly seasonality, light trend changepoints,\\     \# separate holidays +- 4 days, default feature sets and ridge fit algorithm.\\     "DAILY\_SEAS\_NM\_GR\_LINEAR\_CP\_LT\_HOL\_SP4\_FEASET\_AUTO\_ALGO\_RIDGE\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO"\\ {]}\end{tabular}          \\ \hline
%    \multirow{3}{*}{Weekly}                                   & 1                                                                                     & \begin{tabular}[c]{@{}l@{}}SILVERKITE\_WEEKLY = {[}\\     \# For weekly data, normal seasonality up to yearly, no trend changepoints,\\     \# no holiday, no feature sets and linear fit algorithm.\\     "WEEKLY\_SEAS\_NM\_GR\_LINEAR\_CP\_NONE\_HOL\_NONE\_FEASET\_OFF\_ALGO\_LINEAR\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO",\\     \# For weekly data, normal seasonality up to yearly, light trend changepoints,\\     \# no holiday, no feature sets and linear fit algorithm.\\     "WEEKLY\_SEAS\_NM\_GR\_LINEAR\_CP\_LT\_HOL\_NONE\_FEASET\_OFF\_ALGO\_LINEAR\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO",\\     \# For weekly data, heavy seasonality up to yearly, normal trend changepoints,\\     \# no holiday, no feature sets and ridge fit algorithm.\\     "WEEKLY\_SEAS\_HV\_GR\_LINEAR\_CP\_NM\_HOL\_NONE\_FEASET\_OFF\_ALGO\_RIDGE\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO",\\     \# For weekly data, heavy seasonality up to yearly, light trend changepoints,\\     \# no holiday, no feature sets and ridge fit algorithm.\\     "WEEKLY\_SEAS\_HV\_GR\_LINEAR\_CP\_LT\_HOL\_NONE\_FEASET\_OFF\_ALGO\_RIDGE\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO"\\ {]}\end{tabular}                                                                                               \\ \cline{2-3}
%                                                              & 4                                                                                     & \begin{tabular}[c]{@{}l@{}}SILVERKITE\_WEEKLY = {[}\\     \# For weekly data, normal seasonality up to yearly, no trend changepoints,\\     \# no holiday, no feature sets and linear fit algorithm.\\     "WEEKLY\_SEAS\_NM\_GR\_LINEAR\_CP\_NONE\_HOL\_NONE\_FEASET\_OFF\_ALGO\_LINEAR\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO",\\     \# For weekly data, normal seasonality up to yearly, light trend changepoints,\\     \# no holiday, no feature sets and linear fit algorithm.\\     "WEEKLY\_SEAS\_NM\_GR\_LINEAR\_CP\_LT\_HOL\_NONE\_FEASET\_OFF\_ALGO\_LINEAR\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO",\\     \# For weekly data, heavy seasonality up to yearly, normal trend changepoints,\\     \# no holiday, no feature sets and ridge fit algorithm.\\     "WEEKLY\_SEAS\_HV\_GR\_LINEAR\_CP\_NM\_HOL\_NONE\_FEASET\_OFF\_ALGO\_RIDGE\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO",\\     \# For weekly data, heavy seasonality up to yearly, light trend changepoints,\\     \# no holiday, no feature sets and ridge fit algorithm.\\     "WEEKLY\_SEAS\_HV\_GR\_LINEAR\_CP\_LT\_HOL\_NONE\_FEASET\_OFF\_ALGO\_RIDGE\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO"\\ {]}\end{tabular}                                                                                               \\ \cline{2-3}
%                                                              & 4*3                                                                                   & \begin{tabular}[c]{@{}l@{}}SILVERKITE\_WEEKLY = {[}\\     \# For weekly data, normal seasonality up to yearly, no trend changepoints,\\     \# no holiday, no feature sets and linear fit algorithm.\\     "WEEKLY\_SEAS\_NM\_GR\_LINEAR\_CP\_NONE\_HOL\_NONE\_FEASET\_OFF\_ALGO\_LINEAR\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO",\\     \# For weekly data, normal seasonality up to yearly, light trend changepoints,\\     \# no holiday, no feature sets and linear fit algorithm.\\     "WEEKLY\_SEAS\_NM\_GR\_LINEAR\_CP\_LT\_HOL\_NONE\_FEASET\_OFF\_ALGO\_LINEAR\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO",\\     \# For weekly data, heavy seasonality up to yearly, normal trend changepoints,\\     \# no holiday, no feature sets and ridge fit algorithm.\\     "WEEKLY\_SEAS\_HV\_GR\_LINEAR\_CP\_NM\_HOL\_NONE\_FEASET\_OFF\_ALGO\_RIDGE\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO",\\     \# For weekly data, heavy seasonality up to yearly, light trend changepoints,\\     \# no holiday, no feature sets and ridge fit algorithm.\\     "WEEKLY\_SEAS\_HV\_GR\_LINEAR\_CP\_LT\_HOL\_NONE\_FEASET\_OFF\_ALGO\_RIDGE\_AR\_OFF\_DSI\_AUTO\_WSI\_AUTO"\\ {]}\end{tabular}                                                                                               \\ \hline
    \end{tabular}
    \caption{Silverkite configurations used during benchmarking.}
    \label{tab:benchmark-silverkite-config}
\end{table}

